Coboundary expansion inside Chevalley coset complex HDXs

Recent major results in property testing~\cite{BLM24,DDL24} and PCPs~\cite{BMV24} were unlocked by moving to high-dimensional expanders (HDXs) constructed from $\widetilde{C}_d$-type buildings, rather than the long-known $\widetilde{A}_d$-type ones. At the same time, these building quotient HDXs are not as easy to understand as the more elementary (and more symmetric/explicit) \emph{coset complex} HDXs constructed by Kaufman--Oppenheim~\cite{KO18} (of $A_d$-type) and O'Donnell--Pratt~\cite{OP22} (of $B_d$-, $C_d$-, $D_d$-type). Motivated by these considerations, we study the $B_3$-type generalization of a recent work of Kaufman--Oppenheim~\cite{KO21}, which showed that the $A_3$-type coset complex HDXs have good $1$-coboundary expansion in their links, and thus yield $2$-dimensional topological expanders. The crux of Kaufman--Oppenheim's proof of $1$-coboundary expansion was: (1)~identifying a group-theoretic result by Biss and Dasgupta~\cite{BD01} on small presentations for the $A_3$-unipotent group over~$\mathbb{F}_q$; (2)~``lifting'' it to an analogous result for an $A_3$-unipotent group over polynomial extensions~$\mathbb{F}_q[x]$. For our $B_3$-type generalization, the analogue of~(1) appears to not hold. We manage to circumvent this with a significantly more involved strategy: (1)~getting a computer-assisted proof of vanishing $1$-cohomology of $B_3$-type unipotent groups over~$\mathbb{F}_5$; (2)~developing significant new ``lifting'' technology to deduce the required quantitative $1$-cohomology results in $B_3$-type unipotent groups over $\mathbb{F}_{5^k}[x]$.

==> tables/a3-link.tex <==
\begin{table}
\centering
\begin{tabular}{|*{7}{c|}}
\hline
 & $\El{\alpha}{u}$ & $\El{\beta}{u}$ & $\El{\gamma}{u}$ & $\El{\alpha+\beta}{u}$ & $\El{\beta+\gamma}{u}$ & $\El{\alpha+\beta+\gamma}{u}$ \\ \hline
$\El{\alpha}{t}$ & \CellR{X} & \CellG{$\El{\alpha+\beta}{tu}$} & \CellR{$\Id$} & \CellX{$\Id$} & \CellX{$\El{\alpha+\beta+\gamma}{tu}$} & $\Id$ \\ \hline
$\El{\beta}{t}$ & -- & \CellB{X} & \CellR{$\El{\beta+\gamma}{tu}$} & \CellB{$\Id$} & \CellX{$\Id$} & $\Id$ \\ \hline
$\El{\gamma}{t}$ & -- & -- & \CellX{X} & \CellB{$\El{\alpha+\beta+\gamma}{-tu}$} & \CellX{$\Id$} & $\Id$ \\ \hline
$\El{\alpha+\beta}{t}$ & -- & -- & -- & \CellX{X} & \CellX{$\Id$} & $\Id$ \\ \hline
$\El{\beta+\gamma}{t}$ & -- & -- & -- & -- & \CellX{X} & $\Id$ \\ \hline
\end{tabular}
\caption{The commutation relations within the link of $\delta$ in $A_3$. A cell in row $x$, column $y$, with entry $z$ means that $\Comm{x}{y}=z$; for instance, from the top-left cell, $\Comm{\El{\alpha}{t}}{\El{\beta}{u}} = \El{\alpha+\beta}{tu}$. Colors are used to denote which subgroup a particular commutation relation is contained in: \BoxR denotes the span of $\alpha$ and $\beta$; \BoxB denotes the span of $\beta$ and $\gamma$; \BoxG denotes the span of $\alpha$ and $\gamma$; and \BoxX denotes that a relation is not contained within the span of any subgroup (e.g., it may involve elements which are not present in either subgroup). The below diagonal cells are marked with ``--'' and the diagonal cells with ``X''.}\label{table:a3}
\end{table}

==> tables/b3-link-alpha.tex <==

\begin{sidewaystable}
\centering
\begin{tabular}{|*{8}{c|}}
\hline
 & $\El{\beta}{u}$ & $\El{\psi}{u}$ & $\El{\omega}{u}$ & $\El{\beta+\psi}{u}$ & $\El{\psi+\omega}{u}$ & $\El{\beta+2\psi}{u}$ & $\El{\beta+\psi+\omega}{u}$ \\ \hline
$\El{\beta}{t}$ & X & \CellR{$\El{\beta+\psi}{tu}\El{\beta+2\psi}{tu^2}$} & \CellG{$\Id$} & \CellR{$\Id$} & \CellR{$\El{\beta+\psi+\omega}{tu}$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\psi}{t}$ & -- & X & \CellB{$\El{\psi+\omega}{tu}$} & \CellR{$\El{\beta+2\psi}{2tu}$} & \CellR{$\Id$} & \CellB{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\omega}{t}$ & -- & -- & X & \CellX{$\El{\beta+\psi+\omega}{-2tu}$} & \CellX{$\Id$} & \CellB{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\beta+\psi}{t}$ & -- & -- & -- & X & \CellR{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\psi+\omega}{t}$ & -- & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & X & \CellX{$\Id$} \\ \hline
\end{tabular}
\caption{The commutation relations within the link of $\alpha$ in $B_3$. In the above-diagonal region, a cell in row $x$, column $y$, with entry $z$ means that $\Comm{x}{y}=z$; for instance, from the top-left cell, $\Comm{\El{\beta}{t}}{\El{\psi}{u}} = \El{\beta+\psi}{tu}\El{\beta+2\psi}{tu^2}$. Colors are used to denote which subgroup a particular commutation relation is contained in: \BoxR denotes the span of $\beta$ and $\psi$; \BoxB denotes the span of $\psi$ and $\omega$; \BoxG denotes the span of $\beta$ and $\omega$; and \BoxX denotes that a relation is not contained within the span of any subgroup (e.g., it may involve elements which are not present in either subgroup). The below diagonal cells are marked with ``--'' and the diagonal cells with ``X''.}\label{table:b3:alpha}
\end{sidewaystable}

==> tables/b3-link-omega.tex <==

\begin{sidewaystable}
\centering
{
\tiny
\begin{tabular}{|*{10}{c|}}
\hline
 & $\El{\alpha}{u}$ & $\El{\beta}{u}$ & $\El{\psi}{u}$ & $\El{\alpha+\beta}{u}$ & $\El{\beta+\psi}{u}$ & $\El{\beta+2\psi}{u}$ & $\El{\alpha+\beta+\psi}{u}$ & $\El{\alpha+\beta+2\psi}{u}$ & $\El{\alpha+2\beta+2\psi}{u}$ \\ \hline
$\El{\alpha}{t}$ & X & \CellR{$\El{\alpha+\beta}{tu}$} & \CellG{$\Id$} & \CellR{$\Id$} & \CellX{$\El{\alpha+\beta+\psi}{tu} \El{\alpha+2\beta+2\psi}{tu^2}$} & \CellX{$\El{\alpha+\beta+2\psi}{tu}$} & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\beta}{t}$ & -- & X & \CellB{$\El{\beta+\psi}{tu} \El{\beta+2\psi}{tu^2}$} & \CellR{$\Id$} & \CellB{$\Id$} & \CellB{$\Id$} & \CellX{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{tu}$} & \CellX{$\Id$} \\ \hline
$\El{\psi}{t}$ & -- & -- & X & \CellX{$\El{\alpha+\beta+\psi}{-tu} \El{\alpha+\beta+2\psi}{-t^2u}$} & \CellB{$\El{\beta+2\psi}{2tu}$} & \CellB{$\Id$} & \CellX{$\El{\alpha+\beta+2\psi}{2tu}$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\alpha+\beta}{t}$ & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{-tu}$} & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\beta+\psi}{t}$ & -- & -- & -- & -- & X & \CellB{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{2tu}$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\alpha+\beta+\psi}{t}$ & -- & -- & -- & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
$\El{\alpha+\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & -- & -- & X & \CellX{$\Id$} \\ \hline
$\El{\alpha+2\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & -- & -- & -- & X \\ \hline
\end{tabular}
}
\caption{The commutation relations within the link of $\omega$ in $B_3$. In the above-diagonal region, a cell in row $x$, column $y$, with entry $z$ means that $\Comm{x}{y}=z$; for instance, from the top-left cell, $\Comm{\El{\alpha}{t}}{\El{\beta}{u}} = \El{\alpha+\beta}{tu}$. Colors are used to denote which subgroup a particular commutation relation is contained in: \BoxR denotes the span of $\alpha$ and $\beta$; \BoxB denotes the span of $\beta$ and $\psi$; \BoxG denotes the span of $\alpha$ and $\psi$; and \BoxX denotes that a relation is not contained within the span of any subgroup (e.g., it may involve elements which are not present in either subgroup). The below diagonal cells are marked with ``--'' and the diagonal cells with ``X''.}\label{table:b3:omega}
\end{sidewaystable}

% \begin{tabular}{|*{10}{c|}}
% \hline
%  & $\alpha$ & $\beta$ & $\psi$ & $\alpha+\beta$ & $\beta+\psi$ & $\beta+2\psi$ & $\alpha+\beta+\psi$ & $\alpha+\beta+2\psi$ & $\alpha+2\beta+2\psi$ \\ \hline\hline
% $\alpha$ & X & S & S & S & M & M & M & M & M \\ \hline
% $\beta$ & -- & X & S & S & S & S & M & M & M \\ \hline
% $\psi$ & -- & -- & X & M & S & S & M & M & M \\ \hline
% $\alpha+\beta$ & -- & -- & -- & X & M & & M & M & M \\ \hline
% $\beta+\psi$ & -- & -- & -- & -- & X & S & M & M & M \\ \hline
% $\beta+2\psi$ & -- & -- & -- & -- & -- & X & M & M & M \\ \hline
% $\alpha+\beta+\psi$ & -- & -- & -- & -- & -- & -- & X & M & M \\ \hline
% $\alpha+\beta+2\psi$ & -- & -- & -- & -- & -- & -- & -- & X & M \\ \hline
% $\alpha+2\beta+2\psi$ & -- & -- & -- & -- & -- & -- & -- & -- & X \\ \hline
% \end{tabular}


% \begin{sidewaystable}
% \centering
% {
% \tiny
% \begin{tabular}{|*{10}{c|}}
% \hline
%  & $\El{\alpha}{u}$ & $\El{\beta}{u}$ & $\El{\psi}{u}$ & $\El{\alpha+\beta}{u}$ & $\El{\beta+\psi}{u}$ & $\El{\beta+2\psi}{u}$ & $\El{\alpha+\beta+\psi}{u}$ & $\El{\alpha+\beta+2\psi}{u}$ & $\El{\alpha+2\beta+2\psi}{u}$ \\ \hline
% $\El{\alpha}{t}$ & X & \CellR{$\El{\alpha+\beta}{tu}$} & \CellG{$\Id$} & \CellR{$\Id$} & \CellX{$\El{\alpha+\beta+\psi}{tu} \El{\alpha+2\beta+2\psi}{tu^2}$} & \CellX{$\El{\alpha+\beta+2\psi}{tu}$} & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\beta}{t}$ & -- & X & \CellB{$\El{\beta+\psi}{tu} \El{\beta+2\psi}{tu^2}$} & \CellR{$\Id$} & \CellB{$\Id$} & \CellB{$\Id$} & \CellX{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{tu}$} & \CellX{$\Id$} \\ \hline
% $\El{\psi}{t}$ & -- & -- & X & \CellX{$\El{\alpha+\beta+\psi}{-tu} \El{\alpha+\beta+2\psi}{-t^2u}$} & \CellB{$\El{\beta+2\psi}{2tu}$} & \CellB{$\Id$} & \CellX{$\El{\alpha+\beta+2\psi}{2tu}$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\alpha+\beta}{t}$ & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{-tu}$} & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\beta+\psi}{t}$ & -- & -- & -- & -- & X & \CellB{$\Id$} & \CellX{$\El{\alpha+2\beta+2\psi}{2tu}$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\alpha+\beta+\psi}{t}$ & -- & -- & -- & -- & -- & -- & X & \CellX{$\Id$} & \CellX{$\Id$} \\ \hline
% $\El{\alpha+\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & -- & -- & X & \CellX{$\Id$} \\ \hline
% $\El{\alpha+2\beta+2\psi}{t}$ & -- & -- & -- & -- & -- & -- & -- & -- & X \\ \hline
% \end{tabular}
% }
% \caption{The commutation relations within the link of $\omega$ in $B_3$. In the above-diagonal region, a cell in row $x$, column $y$, with entry $z$ means that $\Comm{x}{y}=z$; for instance, from the top-left cell, $\Comm{\El{\alpha}{t}}{\El{\beta}{u}} = \El{\alpha+\beta}{tu}$. Colors are used to denote which subgroup a particular commutation relation is contained in: \BoxR denotes the span of $\alpha$ and $\beta$; \BoxB denotes the span of $\beta$ and $\psi$; \BoxG denotes the span of $\alpha$ and $\psi$; and \BoxX denotes that a relation is not contained within the span of any subgroup (e.g., it may involve elements which are not present in either subgroup). The below diagonal cells are marked with ``--'' and the diagonal cells with ``X''.}\label{table:b3:omega}
% \end{sidewaystable}
